Efficient Video Compression via Content-Adaptive Super-Resolution

Video compression is a critical component of Internet video delivery. Recent work has shown that deep learning techniques can rival or outperform human-designed algorithms, but these methods are significantly less compute and power-efficient than existing codecs. This paper presents a new approach that augments existing codecs with a small, content-adaptive super-resolution model that significantly boosts video quality. Our method, SRVC, encodes video into two bitstreams: (i) a content stream, produced by compressing downsampled low-resolution video with the existing codec, (ii) a model stream, which encodes periodic updates to a lightweight super-resolution neural network customized for short segments of the video. SRVC decodes the video by passing the decompressed low-resolution video frames through the (time-varying) super-resolution model to reconstruct high-resolution video frames. Our results show that to achieve the same PSNR, SRVC requires 16% of the bits-per-pixel of H.265 in slow mode, and 2% of the bits-per-pixel of DVC, a recent deep learning-based video compression scheme. SRVC runs at 90 frames per second on a NVIDIA V100 GPU.

==> Makefile <==
.PHONY: all clean dist print

P = paper

default : $P.pdf

$P.dvi	: $(wildcard *.tex sections/*.tex *.bib figures/*.eps)
	latex  $P < /dev/null || $(RM) $@
	bibtex $P < /dev/null || $(RM) $@
	latex  $P < /dev/null || $(RM) $@
	latex  $P < /dev/null || $(RM) $@

onerun  : $(wildcard *.tex sections/*.tex *.bib figures/*)
	bibtex $P
	pdflatex --shell-escape $P

$P.pdf  : $(wildcard *.tex sections/*.tex *.bib figures/*)
	pdflatex --shell-escape $P
	bibtex $P
	pdflatex --shell-escape $P
	pdflatex --shell-escape $P
	
embedded:
	gs -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -dPDFSETTINGS=/prepress \
	    -dEmbedAllFonts=true \
	    -sOutputFile=$P_embedded.pdf \
	    -f $P.pdf

$P.ps	: $P.dvi
	dvips -tletter -Ppdf $P.dvi -o $P.ps
	ps2pdf -dPDFSETTINGS=/prepress -dEmbedAllFonts=true $P.ps

$P.ps.gz: $P.ps
	$(RM) $P.ps.gz
	gzip -9 < $P.ps > $P.ps.gz

print:	$P.ps

dist:	$P.ps.gz

clean:
	$(RM) $P.pdf $P.log $P.aux $P.bbl $P.blg $P.out $P.dvi $P.ps $P.ps.gz texput.log $P_embedded.pdf

